SilverSpeak: Evading AI-Generated Text Detectors using Homoglyphs

The advent of Large Language Models (LLMs) has enabled the generation of text that increasingly exhibits human-like characteristics. As the detection of such content is of significant importance, substantial research has been conducted with the objective of developing reliable AI-generated text detectors. These detectors have demonstrated promising results on test data, but recent research has revealed that they can be circumvented by employing different techniques. In this paper, we present homoglyph-based attacks (A $\rightarrow$ Cyrillic A) as a means of circumventing existing detectors. We conduct a comprehensive evaluation to assess the effectiveness of these attacks on seven detectors, including ArguGPT, Binoculars, DetectGPT, Fast-DetectGPT, Ghostbuster, OpenAI's detector, and watermarking techniques, on five different datasets. Our findings demonstrate that homoglyph-based attacks can effectively circumvent state-of-the-art detectors, leading them to classify all texts as either AI-generated or human-written (decreasing the average Matthews Correlation Coefficient from 0.64 to -0.01). Through further examination, we extract the technical justification underlying the success of the attacks, which varies across detectors. Finally, we discuss the implications of these findings and potential defenses against such attacks.

==> result_tables/results_table_arguGPT_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.94 & 0.97 & 0.97 & 0.96 & 0.98 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline

\end{tabular}
\caption{Results for \detector{ArguGPT} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_arguGPT_cheat}
\end{table*}


==> result_tables/results_table_arguGPT_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.92 & 0.96 & 0.96 & 0.95 & 0.96 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline

\end{tabular}
\caption{Results for \detector{ArguGPT} on the \dataset{essay} dataset.}
\label{tab:result_table_arguGPT_essay}
\end{table*}


==> result_tables/results_table_arguGPT_realnewslike.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{ArguGPT} on the \dataset{realnewslike} dataset.}
\label{tab:result_table_arguGPT_realnewslike}
\end{table*}


==> result_tables/results_table_arguGPT_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.92 & 0.96 & 0.96 & 0.95 & 0.97 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline

\end{tabular}
\caption{Results for \detector{ArguGPT} on the \dataset{reuter} dataset.}
\label{tab:result_table_arguGPT_reuter}
\end{table*}


==> result_tables/results_table_arguGPT_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.39 & 0.63 & 0.42 & 0.26 & 1.0 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline

\end{tabular}
\caption{Results for \detector{ArguGPT} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_arguGPT_writing_prompts}
\end{table*}


==> result_tables/results_table_binoculars_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.93 & 0.96 & 0.96 & 0.94 & 0.99 \\ \hline
5\% & 0.37 & 0.62 & 0.39 & 0.24 & 1.0 \\ \hline
10\% & 0.11 & 0.51 & 0.05 & 0.03 & 1.0 \\ \hline
15\% & 0.04 & 0.5 & 0.01 & 0.0 & 1.0 \\ \hline
20\% & 0.02 & 0.5 & 0.0 & 0.0 & 1.0 \\ \hline
Greedy & 0.13 & 0.52 & 0.11 & 0.06 & 0.84 \\ \hline

\end{tabular}
\caption{Results for \detector{Binoculars} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_binoculars_cheat}
\end{table*}


==> result_tables/results_table_binoculars_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.91 & 0.95 & 0.95 & 0.9 & 1.0 \\ \hline
5\% & 0.22 & 0.55 & 0.17 & 0.1 & 1.0 \\ \hline
10\% & 0.05 & 0.5 & 0.01 & 0.01 & 1.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.05 & 0.5 & 0.02 & 0.01 & 0.82 \\ \hline

\end{tabular}
\caption{Results for \detector{Binoculars} on the \dataset{essay} dataset.}
\label{tab:result_table_binoculars_essay}
\end{table*}


==> result_tables/results_table_binoculars_realnewslike.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Binoculars} on the \dataset{realnewslike} dataset.}
\label{tab:result_table_binoculars_realnewslike}
\end{table*}


==> result_tables/results_table_binoculars_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.8 & 0.89 & 0.88 & 0.78 & 1.0 \\ \hline
5\% & 0.22 & 0.55 & 0.17 & 0.09 & 1.0 \\ \hline
10\% & 0.07 & 0.51 & 0.02 & 0.01 & 1.0 \\ \hline
15\% & 0.03 & 0.5 & 0.0 & 0.0 & 1.0 \\ \hline
20\% & 0.02 & 0.5 & 0.0 & 0.0 & 1.0 \\ \hline
Greedy & 0.08 & 0.51 & 0.03 & 0.02 & 0.94 \\ \hline

\end{tabular}
\caption{Results for \detector{Binoculars} on the \dataset{reuter} dataset.}
\label{tab:result_table_binoculars_reuter}
\end{table*}


==> result_tables/results_table_binoculars_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.85 & 0.92 & 0.91 & 0.84 & 1.0 \\ \hline
5\% & 0.2 & 0.54 & 0.14 & 0.08 & 1.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & -0.04 & 0.5 & 0.01 & 0.0 & 0.23 \\ \hline

\end{tabular}
\caption{Results for \detector{Binoculars} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_binoculars_writing_prompts}
\end{table*}


==> result_tables/results_table_detectGPT_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.14 & 0.52 & 0.08 & 0.04 & 0.95 \\ \hline
5\% & -0.02 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.03 & 0.51 & 0.13 & 0.08 & 0.55 \\ \hline
15\% & 0.13 & 0.56 & 0.59 & 0.62 & 0.56 \\ \hline
20\% & 0.06 & 0.52 & 0.64 & 0.86 & 0.51 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{DetectGPT} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_detectGPT_cheat}
\end{table*}


==> result_tables/results_table_detectGPT_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.24 & 0.55 & 0.2 & 0.11 & 0.99 \\ \hline
5\% & -0.01 & 0.5 & 0.0 & 0.0 & 0.33 \\ \hline
10\% & 0.11 & 0.53 & 0.16 & 0.09 & 0.72 \\ \hline
15\% & 0.21 & 0.59 & 0.67 & 0.85 & 0.56 \\ \hline
20\% & 0.08 & 0.51 & 0.67 & 0.99 & 0.51 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{DetectGPT} on the \dataset{essay} dataset.}
\label{tab:result_table_detectGPT_essay}
\end{table*}


==> result_tables/results_table_detectGPT_realnewslike.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{DetectGPT} on the \dataset{realnewslike} dataset.}
\label{tab:result_table_detectGPT_realnewslike}
\end{table*}


==> result_tables/results_table_detectGPT_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.23 & 0.56 & 0.22 & 0.12 & 0.93 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.03 & 0.5 & 0.01 & 0.0 & 0.8 \\ \hline
15\% & 0.34 & 0.67 & 0.63 & 0.57 & 0.7 \\ \hline
20\% & 0.14 & 0.54 & 0.67 & 0.94 & 0.52 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{DetectGPT} on the \dataset{reuter} dataset.}
\label{tab:result_table_detectGPT_reuter}
\end{table*}


==> result_tables/results_table_detectGPT_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.44 & 0.68 & 0.55 & 0.39 & 0.93 \\ \hline
5\% & 0.04 & 0.5 & 0.01 & 0.0 & 1.0 \\ \hline
10\% & 0.01 & 0.5 & 0.09 & 0.05 & 0.52 \\ \hline
15\% & 0.02 & 0.51 & 0.57 & 0.65 & 0.51 \\ \hline
20\% & 0.02 & 0.51 & 0.66 & 0.96 & 0.5 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{DetectGPT} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_detectGPT_writing_prompts}
\end{table*}


==> result_tables/results_table_fastDetectGPT_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.9 & 0.95 & 0.95 & 0.94 & 0.95 \\ \hline
5\% & 0.23 & 0.55 & 0.19 & 0.1 & 0.99 \\ \hline
10\% & 0.04 & 0.5 & 0.01 & 0.0 & 1.0 \\ \hline
15\% & 0.02 & 0.5 & 0.0 & 0.0 & 1.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & -0.01 & 0.5 & 0.13 & 0.07 & 0.48 \\ \hline

\end{tabular}
\caption{Results for \detector{Fast-DetectGPT} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_fastDetectGPT_cheat}
\end{table*}


==> result_tables/results_table_fastDetectGPT_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.88 & 0.94 & 0.94 & 0.89 & 0.99 \\ \hline
5\% & 0.22 & 0.55 & 0.2 & 0.12 & 0.93 \\ \hline
10\% & 0.04 & 0.5 & 0.01 & 0.0 & 1.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & -0.08 & 0.48 & 0.08 & 0.04 & 0.35 \\ \hline

\end{tabular}
\caption{Results for \detector{Fast-DetectGPT} on the \dataset{essay} dataset.}
\label{tab:result_table_fastDetectGPT_essay}
\end{table*}


==> result_tables/results_table_fastDetectGPT_realnewslike.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Fast-DetectGPT} on the \dataset{realnewslike} dataset.}
\label{tab:result_table_fastDetectGPT_realnewslike}
\end{table*}


==> result_tables/results_table_fastDetectGPT_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.92 & 0.96 & 0.96 & 0.92 & 1.0 \\ \hline
5\% & 0.28 & 0.57 & 0.25 & 0.14 & 1.0 \\ \hline
10\% & 0.1 & 0.51 & 0.04 & 0.02 & 1.0 \\ \hline
15\% & 0.02 & 0.5 & 0.0 & 0.0 & 1.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.04 & 0.51 & 0.11 & 0.06 & 0.58 \\ \hline

\end{tabular}
\caption{Results for \detector{Fast-DetectGPT} on the \dataset{reuter} dataset.}
\label{tab:result_table_fastDetectGPT_reuter}
\end{table*}


==> result_tables/results_table_fastDetectGPT_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.79 & 0.89 & 0.88 & 0.81 & 0.97 \\ \hline
5\% & 0.3 & 0.59 & 0.31 & 0.19 & 0.96 \\ \hline
10\% & 0.05 & 0.5 & 0.02 & 0.01 & 0.83 \\ \hline
15\% & -0.03 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.5 \\ \hline
Greedy & -0.33 & 0.37 & 0.09 & 0.07 & 0.17 \\ \hline

\end{tabular}
\caption{Results for \detector{Fast-DetectGPT} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_fastDetectGPT_writing_prompts}
\end{table*}


==> result_tables/results_table_ghostbusterAPI_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.64 & 0.8 & 0.83 & 0.99 & 0.71 \\ \hline
5\% & 0.41 & 0.69 & 0.63 & 0.53 & 0.79 \\ \hline
10\% & 0.32 & 0.61 & 0.71 & 0.97 & 0.57 \\ \hline
15\% & 0.12 & 0.52 & 0.67 & 1.0 & 0.51 \\ \hline
20\% & 0.06 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline
Greedy & 0.02 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{Ghostbuster} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_ghostbusterAPI_cheat}
\end{table*}


==> result_tables/results_table_ghostbusterAPI_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.92 & 0.96 & 0.96 & 0.95 & 0.96 \\ \hline
5\% & 0.73 & 0.86 & 0.84 & 0.76 & 0.94 \\ \hline
10\% & 0.51 & 0.71 & 0.77 & 0.99 & 0.64 \\ \hline
15\% & 0.13 & 0.52 & 0.67 & 1.0 & 0.51 \\ \hline
20\% & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{Ghostbuster} on the \dataset{essay} dataset.}
\label{tab:result_table_ghostbusterAPI_essay}
\end{table*}


==> result_tables/results_table_ghostbusterAPI_realnewslike.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Ghostbuster} on the \dataset{realnewslike} dataset.}
\label{tab:result_table_ghostbusterAPI_realnewslike}
\end{table*}


==> result_tables/results_table_ghostbusterAPI_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.93 & 0.96 & 0.96 & 0.94 & 0.99 \\ \hline
5\% & 0.61 & 0.79 & 0.75 & 0.63 & 0.93 \\ \hline
10\% & 0.51 & 0.72 & 0.78 & 0.98 & 0.64 \\ \hline
15\% & 0.16 & 0.53 & 0.68 & 1.0 & 0.51 \\ \hline
20\% & 0.04 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{Ghostbuster} on the \dataset{reuter} dataset.}
\label{tab:result_table_ghostbusterAPI_reuter}
\end{table*}


==> result_tables/results_table_ghostbusterAPI_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.88 & 0.94 & 0.94 & 0.9 & 0.98 \\ \hline
5\% & 0.42 & 0.66 & 0.49 & 0.33 & 0.96 \\ \hline
10\% & 0.64 & 0.82 & 0.83 & 0.86 & 0.79 \\ \hline
15\% & 0.33 & 0.6 & 0.71 & 0.99 & 0.56 \\ \hline
20\% & 0.09 & 0.51 & 0.67 & 1.0 & 0.5 \\ \hline
Greedy & 0.0 & 0.5 & 0.67 & 1.0 & 0.5 \\ \hline

\end{tabular}
\caption{Results for \detector{Ghostbuster} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_ghostbusterAPI_writing_prompts}
\end{table*}


==> result_tables/results_table_openAIDetector_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.47 & 0.7 & 0.61 & 0.46 & 0.9 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & -0.02 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
Greedy & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline

\end{tabular}
\caption{Results for \detector{OpenAI} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_openAIDetector_cheat}
\end{table*}


==> result_tables/results_table_openAIDetector_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & -0.21 & 0.43 & 0.09 & 0.06 & 0.22 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.5 \\ \hline
Greedy & 0.03 & 0.5 & 0.0 & 0.0 & 1.0 \\ \hline

\end{tabular}
\caption{Results for \detector{OpenAI} on the \dataset{essay} dataset.}
\label{tab:result_table_openAIDetector_essay}
\end{table*}


==> result_tables/results_table_openAIDetector_realnewslike.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{OpenAI} on the \dataset{realnewslike} dataset.}
\label{tab:result_table_openAIDetector_realnewslike}
\end{table*}


==> result_tables/results_table_openAIDetector_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & 0.27 & 0.57 & 0.25 & 0.14 & 0.98 \\ \hline
5\% & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & -0.04 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & -0.09 & 0.49 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & -0.11 & 0.49 & 0.0 & 0.0 & 0.06 \\ \hline
Greedy & -0.06 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline

\end{tabular}
\caption{Results for \detector{OpenAI} on the \dataset{reuter} dataset.}
\label{tab:result_table_openAIDetector_reuter}
\end{table*}


==> result_tables/results_table_openAIDetector_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline
Original & -0.05 & 0.5 & 0.0 & 0.0 & 0.11 \\ \hline
5\% & -0.04 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
10\% & -0.05 & 0.5 & 0.0 & 0.0 & 0.0 \\ \hline
15\% & -0.13 & 0.48 & 0.0 & 0.0 & 0.0 \\ \hline
20\% & -0.11 & 0.49 & 0.01 & 0.0 & 0.11 \\ \hline
Greedy & 0.01 & 0.5 & 0.01 & 0.0 & 0.57 \\ \hline

\end{tabular}
\caption{Results for \detector{OpenAI} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_openAIDetector_writing_prompts}
\end{table*}


==> result_tables/results_table_watermark_cheat.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Watermark} on the \dataset{CHEAT} dataset.}
\label{tab:result_table_watermark_cheat}
\end{table*}


==> result_tables/results_table_watermark_essay.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Watermark} on the \dataset{essay} dataset.}
\label{tab:result_table_watermark_essay}
\end{table*}


==> result_tables/results_table_watermark_reuter.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Watermark} on the \dataset{reuter} dataset.}
\label{tab:result_table_watermark_reuter}
\end{table*}


==> result_tables/results_table_watermark_writing_prompts.tex <==

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Type} & \textbf{MCC} & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} \\ \hline

\end{tabular}
\caption{Results for \detector{Watermark} on the \dataset{writing prompts} dataset.}
\label{tab:result_table_watermark_writing_prompts}
\end{table*}

